Smooth ECE: Principled Reliability Diagrams via Kernel Smoothing

Calibration measures and reliability diagrams are two fundamental tools for measuring and interpreting the calibration of probabilistic predictors. Calibration measures quantify the degree of miscalibration, and reliability diagrams visualize the structure of this miscalibration. However, the most common constructions of reliability diagrams and calibration measures -- binning and ECE -- both suffer from well-known flaws (e.g. discontinuity). We show that a simple modification fixes both constructions: first smooth the observations using an RBF kernel, then compute the Expected Calibration Error (ECE) of this smoothed function. We prove that with a careful choice of bandwidth, this method yields a calibration measure that is well-behaved in the sense of (B{\l}asiok, Gopalan, Hu, and Nakkiran 2023a) -- a consistent calibration measure. We call this measure the SmoothECE. Moreover, the reliability diagram obtained from this smoothed function visually encodes the SmoothECE, just as binned reliability diagrams encode the BinnedECE. We also provide a Python package with simple, hyperparameter-free methods for measuring and plotting calibration: `pip install relplot\`.

==> _intro1.tex <==
\section{Introduction}

\begin{figure}[th]
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{code/figures/basic_binned.png}
         % \caption{Traditional reliability diagram.}
         \label{fig:old}
     \end{subfigure}\hspace{2cm}%
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{code/figures/hero.png}
         % \caption{Proposed reliability diagram (one instance in a family)}
         \label{fig:new}
     \end{subfigure}
     \caption{{\bf Left:} Traditional reliability diagram based on binning, which 
     is equivalent to histogram regression.
     {\bf Right:} An example of the proposed reliability diagram, based on more sophisticated
     regressors (in this case, kernel smoothing).
     \pnote{todo: add ECE and intCE labels to left/right. Do opacity on main line on right. Also, use CV to find optimal kde bandwidth for the density plots}
     }
\end{figure}


\emph{Reliability diagrams} are tools to visualize the calibration of predictors.
While calibration metrics (e.g. ECE, dCE) quantify the overall amount of miscalibration,
reliability diagrams are meant to convey the \emph{structure} of this miscalibration---e.g. on which outputs the predictor is over- or under-confident, and by how much.
In a weather forecasting setting for example,
if it actually rains on only 60\% of the days for which 
a certain forecaster predicts a 90\% chance of rain, then this forecaster is overconfident
on their 90\% predictions, which we would like to see revealed in a reliability diagram.
The traditional goal of reliability diagrams is to
estimate these conditional probabilities, e.g. the true probability of rain
given the forecaster predicts a 90\% chance of rain.
This goal is formally equivalent to the goal of statistical regression---
an equivalence that is both trivial and known, but not fully appreciated in the current literature.

To elaborate, %#on the regression perspective and its benefits,
it is helpful to introduce some notation.
We have a binary classifier $f$ producing probabilities $f(x) \in [0, 1]$.
We are given iid samples of prediction and observation pairs:
$\{(f(x_i), y_i)\}_{(x_i, y_i) \sim \cD}$ where $y_i \in \{0, 1\}$.
% For example, set of rain forecasts $\{f(x_i)\}$ and observations of rain $\{y_i\}$.
For example, the rain forecast $f(x_i)$ and
the corresponding actual observation of rain $y_i \in \{0, 1\}$.
We want to estimate the true conditional density function
$\mu(\ell) := \E_{(x, y) \sim \cD}[ y \mid f(x)=\ell]$.
The plot of our estimate of $\mu: [0, 1] \to [0, 1]$ is what we call a \emph{reliability diagram}.
A perfectly calibrated classifier will have $\mu(\ell) = \ell$,
and thus a diagonal reliability diagram.

With the above setup, it is clear that 
constructing a reliability diagram is simply a 1-dimensional regression problem.
After all, our goal is to estimate the conditional $\mu(f) = \E[y \mid f]$
given iid samples $(f_i, y_i) \in \R \x \R$, where we let $f_i := f(x_i)$.
This is exactly the objective of regressing $y \in \R$ on $f \in \R$.
% Thus, methods to estimate reliability diagrams are exactly regression methods.
Thus, all regression methods yield a corresponding method of constructing reliability diagrams:
the popular practice of ``binning'' reliability diagrams, for example,
exactly corresponds to the histogram-estimator in statistics,
which fits a family of piecewise-constant functions to $\mu(f)$\footnote{To be concrete, the binned reliability diagram is equivalent to
the regression estimate $\hat{\mu}(f)$
over the family of piecewise-constant step functions:
\begin{equation}
\label{eqn:simple}
\hat{\mu}
=
\argmin_{g \in \cF_{\textrm{bin}(k)}}
\E_{(f, y)}[ ||g(f) - y||^2 ]
\end{equation}
with the family of functions
$\cF_{\textrm{bin}(k)} = \{ g(x) = \sum_i \alpha_i \1\{x \in \mathrm{Bin}_i\}  \mid \alpha_1, \dots \alpha_k \in \R \}$
where $\{\mathrm{Bin}_1, \dots, \mathrm{Bin}_k\}$ is a partition of the unit interval into $k$ regular intervals.
The optima here is achieved at $\alpha_i = \E[y \mid f \in \mathrm{Bin}_i]$.}.

The connection to regression has been noted in the literature (e.g. \citet{brocker2008some}),
but the lessons from statistical regression have not caught on in estimating reliability diagrams.
For example, from the statistical perspective, histogram estimation (``binning'') is a fairly naive
method of regression, and can often be improved on by more sophisticated methods
(e.g. kernel smoothing, kernel ridge regression, isotonic regression, etc).
Yet binning has long been the de-facto standard for computing reliability diagrams
\citep{murphy1977reliability,degroot1983comparison},
and continues to be used by the machine learning community, including in the GPT-4 tech report \citep{zadrozny2001obtaining,niculescu2005predicting,guo2017calibration,nixon2019measuring,minderer2021revisiting,desai2020calibration,openai2023gpt4}.
In several of these works, binning is even taken as the definition of a reliability diagram
(which conflates the estimand with the estimation procedure).

% And when binning is used,
% there is much debate about how to best choose the bin-widths---
% it is well-known that binned reliability diagrams
% are very sensitive to this choice, which can change conclusions
% about calibration.
And when binning is used,
there is much debate about how to best choose the bin-widths---
a parameter which can severely affect the resulting reliability diagram.
% it is well-known that binned reliability diagrams
% are very sensitive to this choice, which can change conclusions
% about calibration.
On the other hand, the regression perspective provides a concrete prescription:
the objective of regression is to minimize test loss, and so the optimal
hyperparameters are those which minimize test loss (e.g. as measured with a holdout set).
Translated to reliability diagrams, this means the optimal choice of bin-width is
the one with smallest $\mathcal{L}_2$ test loss\footnote{Any proper loss would suffice.},
as measured on a holdout set.
This strategy for picking bin-widths implicitly addresses the popular concerns:
it balances the estimation-error from picking too large bins with the generalization-error from picking too small bins.
After all, these are the same concerns we have in regression.
This strategy has been suggested before \citep{brocker2008some}, though it does not appear to be appreciated
in much of the calibration literature.
We show some examples of this binning strategy in \pnote{todo, maybe inline fig}.

% For example, the regression perspective suggests concrete improvements to
% the practice of binning.

% as simply one of many possible estimators for the underlying object.


% This connection between reliability diagrams and regression is mathematically trivial,
% but does not appear to be fully exploited in the literature.

% There is much discussion about how to pick the bin-widths used in binning.
% for ``binning''-based reliability diagrams, and how care must be taken in choosing bin-width because of this.

We can imagine at least two reasons why the methods of statistical regression have not taken hold
in constructing reliability diagrams.
% We can imagine at least two factors preventing the methods of statistical regression 
% from taking hold in practical studies of reliability diagrams.
% from have not taken hold
% in constructing reliability diagrams in practice.
First, convenience: binning is easy to implement, intuitive to understand, and the obvious implementation runs in linear-time.
These properties are not always true of more sophisticated methods.
Second, the vast design space of other regression methods:
performing a regression involves many experimental choices (e.g. choice of method, kernel, regularization, etc),
which ideally should be informed by our assumptions and priors
about the underlying ground-truth $\mu(f)$, such as smoothness, monotonicity, etc.
It is not always clear how to make these choices, and so the experimenter
may prefer a tool that does not afford them such choices, and 
requires minimal assumptions about the data.

% More generally, once we are doing regression,
% we are free to choose our regression method.
% The histogram estimator is a particularly naive method of regression,
% so we should expect to do better with other standard methods
% (such as kernel smoothing, kernel ridge regression, isotonic regression, etc).
% The choice of regression method for reliability diagrams
% should be informed by our assumptions and priors
% about the underlying ground-truth $\mu(f)$, such as smoothness, monotonicity, etc,
% just as it is in regression.

% In general, different regression methods yield different methods
% for estimating reliability diagrams, inheriting their relative strengths and weaknesses.

% We consider the following setting:
% let $f: \cX \to [0, 1]$ be a binary classifier, which outputs numbers $f(x)$ that we
% interpret as the probability $y=1$ given $x$.
% Let $\cD$ be a ground-truth distribution over input-label pairs $(x, y)$,
% where $x \in \cX$ and $y \in \{0, 1\}$.
% We say the classifier $f$ is \emph{perfectly calibrated} on $\cD$ iff
% $\forall \ell \in [0, 1]: \E[y \mid f(x) = \ell] = \ell$.
% With this setup, the reliability diagram estimation problem is as follows.
% We are given iid samples of prediction-label pairs
% $\{(f(x_i), y_i)\}_{(x_i, y_i) \sim \cD}$,
% and we want to estimate the true conditional density function
% $\mu(\ell) := \E_{(x, y) \sim \cD}[ y \mid f(x)=\ell]$.
% The plot of our estimate of $\mu: [0, 1] \to [0, 1]$ is what we call a \emph{reliability diagram}.
% A perfectly calibrated classifier will have $\mu(\ell) = \ell$,
% and thus a diagonal reliability diagram.

With this User's Guide, we intend to address both factors.
We present a simple, hyperparameter-free regression method that 


Moreover, methods for uncertainty quantification in regression
can be directly ported to quantify uncertainty in reliability diagrams
(e.g. bootstrapping, gaussian process regression, and conformal prediction).



{\bf Contributions.}
We propose a regression-centric perspective on reliability diagrams,
motivated by the simple observation that the goals of regression and reliability diagrams are identical.
This attaches a concrete objective function to reliability diagrams:
they should minimize the regression test loss, with respect to a proper scoring rule.
This principle guides applications of existing methods (such as binning),
and also suggests more powerful methods for constructing reliability diagrams from more powerful regressors.

We give explicit practical suggestions for constructing reliability diagrams.
In particular, we suggest using Nadaraya–Watson kernel regression with a triangular kernel,
and quantifying uncertainty via bootstrapping.
This choice is both interpretable and theoretically justified.
We prove that with a careful choice of bandwidth, this estimator produces functions $\mu$
such that $ECE(\mu) \approx intCE(f(x), y)$.
\pnote{todo, say a bit more about this.} 
We provide code which generates reliability diagrams using our suggestions here: \pnote{todo.}

Moreover, methods for uncertainty quantification in regression
can be directly ported to quantify uncertainty in reliability diagrams
(e.g. bootstrapping, gaussian process regression, and conformal prediction).

% In general, the connection to regression
% attaches a concrete objective function to reliability diagrams:
% they should minimize the regression loss, with respect to any proper scoring rule.

% \pnote{below is scratch:}



% This connection, while trivial, opens up several useful directions:
% \begin{itemize}
%     \item Different regression methods yield different methods for estimating reliability diagrams, inheriting their relative strenghts and weaknesses (eg: isotonic regression, kernel regression, kernel smoothing, logistic regression).
%     \item Methods for selecting hyperparameters in regression yield methods for selecting hyperparms (such as ``bin width'') in reliability diagrams.
%     \item Methods to estimate uncertainty in regression yield methods to estimate uncertainity in reliability diagrams.
% \end{itemize}


% {\bf Generalization.} This connection also clarifies the behavior of reliability diagrams
% at finite sample sizes.
% Much has been written about how finite-sample estimation error poses issues
% for ``binning''-based reliability diagrams, and how care must be taken in choosing bin-width because of this.
% In the regression perspective, this is just the well-known generalization problem: we are optimizing a loss on our ``train set'' of samples $(f_i, y_i)$,
% but we care about our loss on the test distribution
% (the expectation in Equation~\eqref{eqn:simple}),
% so we must be sure our learning method generalizes.
% One way of doing this is by controlling the capacity of our function family (e.g. bin-width),
% another way is by cross-validating with a holdout set.

==> _old_abstract.tex <==
We present practical guidance for constructing theoretically-principled
reliability diagrams, along with a corresponding Python package.

Reliability diagrams are figures used to visualize
the calibration of probabilistic predictions.
Calibration measures, in turn, are functions which quantify
the degree of this calibration.
% While many methods to construct these diagrams have been proposed,
% the classic method of ``binning'' remains the most popular,
% despite its well-known flaws.
The most common constructions of reliability diagrams
and calibration measures --- binning and ECE ---
both suffer from well-known flaws (e.g. discontinuity).
We show that a simple modification fixes both constructions:
simply smooth the observations using an RBF kernel
with a particular bandwidth.
This method yields reliability diagrams
for which the Expected Calibration Error (ECE) of the
smoothed diagram is in
fact a \emph{consistent calibration measure} of the 
original function, in the sense of \citet*{UTC1}.
Our provided Python routine is hyperparameter-free, and runs in quasilinear time.
% \pnote{say "hyperparameter-free" }

% Although many methods to construct these diagrams have been proposed,
% there is no consensus on which method to choose and why.
% To address this, we identify two desiderata of reliability diagrams:
% they should be regression methods (such as histogram binning),
% and they should visually encode a calibration metric (such as ECE).
% Most existing methods, including binning and isotonic regression,
% fall short on at least one front.

% no method has gained traction beyond the standard method of ``binning,''
% which has well-known flaws.
% In absence of a satisfying alternative, 
% what distinguishes these methods

% We show that a certain simple method satisfies both our desiderata:
% Nadaraya-Watson kernel smoothing, with the RBF kernel
% and a careful (automatic) choice of bandwidth.
% This smoothing method yields reliability diagrams
% for which the Expected Calibration Error (ECE) of the diagram
% is in fact a \emph{consistent calibration measure} in the sense of \citet*{UTC1},
% meaning that it provably approximates the
% $\ell_1$ deviation of the classifier from perfect calibration.


% meaning that the true distance from calibration
% can be estimated by simply looking at deviations from the diagonal
% in the reliability diagramo



\iffalse
Reliability diagrams are figures used to quantify and visualize
the calibration of probabilistic predictions.
We present practical guidance for constructing theoretically-principled
reliability diagrams, along with a corresponding Python package.
% We present a Python package for constructing theoretically-principled reliability diagrams,
% along with proofs of its theoretical properties.
% Many methods to construct these diagrams have been proposed, e.g. binning,
% isotonic regression, spline fitting --- but there is still no accepted best-practice,
% and there are well-known problems with even popular methods (such as binning).

In order to construct a good reliability diagram, 
we must ask: what \emph{is} a reliability diagram?
What properties do we want, and how best do we achieve them?
% But what properties do we actually desire in reliability diagrams, and how best do we achieve them?
We identify two natural desiderata of reliability diagrams:
First, they should be regression methods --- and thus reasonable estimates of the true conditional distribution of outcome $y$ given prediction $f(x)$.
Second, they should visually encode a calibration metric (such as ECE).
Most existing methods fall short on at least one front:
the popular method of ``binning,'' for example, is both a
fairly naive regression method, and encodes a poorly-behaved
calibration metric (ECE).


% The arguably most popular method of constructing these diagrams --- binning ---
% suffers from well-known theoretical and practical issues.
% Many alternative methods have been proposed, but none have become standard,
% partly because there is no established criteria to evaluate diagramming methods.


We prove that a certain simple method satisfies both our desiderata:
Nadaraya-Watson kernel smoothing, with the RBF kernel
and a careful (automatic) choice of bandwidth.
% We then give a concrete recommendation of which regressor to use:
% We prove that 
This particular method yields reliability diagrams
for which the Expected Calibration Error (ECE) of the diagram
is in fact a \emph{consistent calibration measure} \citep{UTC1},
meaning that it 

meaning that the true distance from calibration
can be estimated by simply looking at deviations from the diagonal
in the reliability diagram.
% Such a property is intuitively desirable, but subtle: it is not satisfied by e.g. isotonic regression or binning.
\fi

==> intCE.tex <==
\section{Reliability Diagrams from Consistent Calibration Measures}
\label{sec:intCE}

We must now decide which regression method to use.
Any regression method can in theory be used for a reliability diagram,
% Which one should we choose?
and many have been proposed for this purpose,
including: isotonic regression \citep{dimitriadis2020evaluating},
kernel smoothing \citep{zhang2020mix},
spline-fitting \citep{guptacalibration},
boosted GAMs \citep{xenopoulos2022calibrate},
and
LOESS regression \citep{austin2014graphical,steyerberg2008clinical,van2016calibration}.
It is apriori unclear which method we should chose, and why.

\pnote{todo:}

We propose using a method that satisfies an additional property:
informally, the total deviation from diagonal in the resulting reliability diagram
should be a reasonable measure of miscalibration ---
specifically, a \emph{consistent calibration measure} as defined in \citep{UTC1}.

% We are left to chose which regression method to use.

We propose using a method that safisfies the following additional property:
The integrated deviation $\E_f[ |\hat{\mu}(f) - f| ]$ is polynomially-related
to the \emph{calibration distance} \citep{UTC1}.
Intuitively, we want the ``amount of deviation from the diagonal'' to
reflect the true distance from calibration. This goal is at-odds with $\hat{\mu}$
being a perfect estimator of $\E[ y | f]$, but we can chose how to balence these concerns.

To achieve this, we suggest using a Nataraya-Watson kernel regression (basically a normalized convolution with the kernel $K$), given by the formula 

\subsection{Importance of Consistent Calibration Measures}
Let us consider a potential classifier which on all the positive examples provides a prediction $0.5 + \varepsilon$, and on all negative classifiers provides a prediction $0.5 - \varepsilon$. As $\varepsilon \to 0$, it is arguable that such a predictor should be considered well-calibrated: indeed, it is not meaningfully different than the constant predictor always outputting $0.5$ --- which is perfectly calibrated. Yet, many naive calibration measures (chiefly, binned version of ECE when the number of bins happen to be even), when applied to such a predictor would report the calibration error close to $0.5$.

In \cite{UTC1} the notion of \emph{consistent calibration measure} was defined --- a calibration measure is consistent if it is polynomially related to a perturbation that is necessary in order to transform a given classifier into a perfectly calibrated one. In particular, in the example described above, such a perturbation is on the order of $\varepsilon$ --- it is enough to decrease some predictions by $\varepsilon$ and increase other by $\varepsilon$ to get a perfectly calibrated classifier.

\begin{figure}[!h]
     \centering
     \includegraphics[width=\textwidth]{code/figures/two_points_close.png}
     \label{}
     \caption{The outcome $y$ is $\{0, 1\}$ with equal probabilities. The prediction is always equal to $1/2 + y \varepsilon$. For $\varepsilon = 0.005$, our method compared with reliability diagram produced by choosing the bandwidth via cross-validation, and the binning diagram. The reported intCE calibration error is relatively small, indicating that the predictor is close to calibrated.}
\end{figure}

As it turns out, by carefully choosing the smoothing parameter $\sigma$ we can ensure that the calibration measure given by an $L_1$ norm of the Nataraya-Watson kernel regression on $\mathbb{E}[y - f|f]$ (\emph{the reliability residual}) from the identity function is a consistent calibration measure.

Specifically, let us consider a gaussian kernel $K_{G}(t) = \exp(-t^2/2) / \sqrt{ 2 \pi }$. On the samples $(f_1, y_1), \ldots (f_n, y_n)$ of pairs of  prediction and outcome, we can compute the kernel density estimation of the density $f$ as
\begin{equation*}
    \phi(t) := \frac{1}{n} \sum_i K(t - f_i),
\end{equation*}
and the estimation of the reliability residual curve as a Natara-Watson kernel regression of $\E[y - f | f]$, that is
\begin{equation*}
    \hat{\mu}(t) := \frac{1}{\phi(t)} \frac{1}{n} \sum_i [K(t - f_i) (f_i - y_i)].
\end{equation*}
Our reliability diagrams consist of plotting this density $\phi$ and the estimator $f + \hat{\mu}$. We can naturally associate a visually appealing calibration measure with such a reliability diagram --- we should just consider the average with respect to the estimated density $\phi$ of the estimated deviation $\hat{\mu}$ 
\begin{equation*}
    \mathrm{CE}_{K} := \int |\hat{\mu}(t)| \phi(t) \, \dt.
\end{equation*}

We can expand this entire expression and cancel the $\phi(t)$ with $1/\phi(t)$ term as
\begin{equation}
\label{eq:cek_emp}
    \mathrm{CE}_K = \int |
    \frac{1}{n} \sum_i K(t - f_i) (f_i - y_i)| \dt,
\end{equation}
and more generally for arbitrary distribution of predictions and outcomes $(f,y)$ we can write
\begin{equation}
\label{eq:cek_gen}
    \mathrm{CE}_K =  \int \left| \E_{(f,y)}[K(t - f) (f - y)]\right| \dt.
\end{equation}
The equation~\eqref{eq:cek_emp} is a special case of~\eqref{eq:cek_gen} when applied to the empirical distribution over pairs $(f_i, y_i)$.

Let us now start with a fixed kernel $K$. We can associate with this kernel a single parameter family of scaled kernels $K_\sigma(t) := \sigma K(t/\sigma)$. As it turns out, under relatively weak conditions on the kernel $K$ (satisfied, for example, by the Gaussian kernel or the triangular kernel $K_{\Delta}(t) := \max(0, 1 - |t|)$), the measure $\min_{\sigma} CE_{K_{\sigma}}(f, e) + |\sigma|$ is a consistent calibration measure.

Specifically when the kernel $K$ is a Gaussian kernel, the measure $CE_{\sigma K}(f,y)$ is decreasing as we increase the kernel parameter $\sigma$. In particular, there is a unique $\sigma_*$ such that $CE_{\sigma_* K}(f, y) = \sigma_*$, and it can easily be found with binary search.

\begin{figure}[!h]
     \centering
     \includegraphics[width=\textwidth]{code/figures/two_points_far.png}
     \label{}
     \caption{The outcome $y$ is $\{0, 1\}$ with equal probabilities. The prediction is always equal to $1/2 + y \varepsilon$ for $\varepsilon := 0.2$. The predictors calibration is considerably worse than the previous one, but it is not apparent from the binning diagram, and the ECE measure has in fact improved.}
\end{figure}
\subsection{Our Proposal}

\pnote{include psuedocode of the method? perhaps omitting the choice of bandwidth part.}
\jnote{Sure}

{\bf Claim (TODO)}: Kernel-smoothing with a triangular kernel of appropriate bandwitdh (the width used by intCE) yields an estimator that satisfies the above properties.




==> intro2.tex <==

% \vspace{1cm}
% \begin{figure}[h]
%      \centering
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{code/figures/hero_binned.png}
%          % \caption{Traditional reliability diagram.}
%          \label{fig:old}
%      \end{subfigure}\hspace{2cm}%
%      \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{code/figures/hero.png}
%          % \caption{Proposed reliability diagram (one instance in a family)}
%          \label{fig:new}
%      \end{subfigure}
%      \caption{{\bf Left:} Traditional reliability diagram based on binning, which 
%      is equivalent to histogram regression.
%      {\bf Right:} Proposed reliability diagram based on kernel regression,
%      with our theoretically-justified choice of bandwidth and calibration metric.
%      Plot generated by our Python package \texttt{relplot}.
%      }
%      \label{fig:hero}
% \end{figure}

% \newpage
\section{old-Introduction}
% \input{intro_code}

\pnote{todo: don't start with Rel Diagrams. Include some of the rel works on regression, then show how the issue is subtle.}
\emph{Reliability diagrams} are tools to visualize the calibration of predictors.
While calibration measures such as Expected Calibration Error (ECE) quantify the overall amount of miscalibration,
reliability diagrams are meant to convey the \emph{structure} of this miscalibration---e.g. on which outputs the predictor is over- or under-confident, and by how much.
In a weather forecasting setting for example,
if it actually rains on only 60\% of the days for which 
a certain forecaster predicts a 90\% chance of rain, then this forecaster is overconfident
on their 90\% predictions, which we would like to see revealed in a reliability diagram.
These diagrams are typically constructed via \emph{binning}:
grouping forecasted probabilities into discrete bins
and computing empirical frequencies
within each bin, as shown in Figure~\ref{fig:hero} (left).
For example, a single bin may group days
forecasted to have between 60-70\% chance of rain, and compute the true fraction of rainy days
within this group.
% The traditional goal of reliability diagrams is to estimate
% these conditional probabilities, e.g. the true probability of rain
% given the forecaster predicts a 90\% chance of rain \cite{?}.
% This is usually estimated
% via \emph{binning}: grouping forecasted
% probabilities into discrete bins, and computing expected observations within each bin, as shown in Figure~\ref{fig:hero} (left).
Binning has a long history and is intuitively appealing,
but has well-known flaws, e.g. the resulting diagrams can be very sensitive to the choice of bin widths,
and the associated calibration measure (BinnedECE)
is discontinuous.

In response, many works have proposed alternate methods of constructing reliability diagrams to improve upon binning -- either as variants
of binning or entirely new procedures.
For example, \citet{?}
However, it is not clear how to chose among these methods,
partly because there is no accepted standard
of what makes a ``good'' reliability diagram.
\pnote{While what it means to be good calibration measure has been studied, not so for reliability diagrams}
% And 
% among these methods,
% Among these many options and without clear guidance,
In absence of a clearly better alternative,
binning remains the arguably most popular method in practice.
% despite these more sophisticated proposals.

To clarify this situation,
we suggest the following desiderata.
A good reliability diagram construction should:
\begin{enumerate}
    \item
    {\bf Implement a regression method}
    \item
    {\bf Visually encode a consistent calibration measure} \citep{UTC1}.
    % \item 
    % {\bf Be hyperparameter-free}
\end{enumerate}

% There are of course other desirable aspects of reliability diagrams,
% such as admitting efficient estimation algorithms, but we take these
% as secondary considerations.
We elaborate below.

{\bf 1. Implement a regression method.}
First, observe that binning is a regression method:
% Statistically, binning is a regression method,
it is equivalent to using histogram regression to regress the observations $y \in \{0, 1\}$ (e.g. rain vs. no rain)
against the predictions $f(x) \in [0, 1]$ (forecasted chance of rain, given features $x$),
in order to estimate the regression function $\mu: f(x) \mapsto \E[ y \mid f(x) ]$.
This function $\mu: [0, 1] \to [0, 1]$ encodes the conditional
probability of $y$ given $f$ (e.g. probability of rain given forecasted chance of rain), and is sometimes called the ``ideal reliability curve'' \citep{?}.
% though it is not neccesarily ideal for us.
With this perspective, we see that
binning is just one of many possible regression methods,
and we could chose any other method (e.g. kernel ridge regression, kernel smoothing, isotonic regression) to give reasonable conditional probability estimates.
However, despite the rich toolbox of regression methods at our disposal,
most reliability diagrams still use the fairly naive histogram estimator.
This suggests that users of reliability diagrams have
additional desiderata --- and so the best regression method may not yield the best reliability diagram. This additional desiderata, we posit, is that diagrams must visually encode
a calibration metric.
    
% The goal of reliability diagrams is usually formalized as
% estimating these conditional probabilities, e.g. the true probability of rain
% given the forecaster predicts a 90\% chance of rain \cite{?}.
% This goal is formally equivalent to statistical regression:
% estimating the expected observation, conditioned on predictions\footnote{This fact is not always appreciated in the calibration literature.}.
% However, while the field of statistics has developed a rich toolbox of regression techniques,
% reliability diagrams still often use the most basic technique: histogram regression (``binning'').
% In order to construct a good reliability diagram, 
% we must therefore ask: what \emph{is} a reliability diagram?
% What properties do we want, and how best do we achieve them?

{\bf 2. Visually encode a consistent calibration measure.}
For binning, it is easy to read-off a common measure of calibration (BinnedECE)
by simple visual inspection of the binned reliability diagram.
This is an appealing property in practice, although the particular measure of BinnedECE has flaws.
Instead, we want reliability diagrams to visually encode
a \emph{consistent calibration measure} \citep{UTC1},
which is a measure that is provably well-behaved in a certain sense.
% with certain theoretical guarantees of being well-behaved.
% a ``good'' calibration measure, which 
% this property of diagrams encoding measures 
% This close relation between 
% a close relation between the reliability diagram
% and some calibration measure (not necessarily ECE), 
This requirement rules out many sophisticated regression methods,
which are not accompanied by corresponding calibration measures.
% Note that this property is not always satisfied by more sophisticated regression methods,
% In general, we want reliability diagrams to be accompanied by a corresponding calibration measure (not neccesarily ECE), which can be easily visually decoded from the diagram.



% , and  requires minimal (if any) assumptions about the data.


% We can imagine at least three reasons why the methods of statistical regression have not taken hold
% in reliability diagrams, in contrast to the common practice of binning.
% \begin{enumerate}
%     \item Practical convenience: binning is easy to implement, intuitive to understand, and the obvious implementation runs in linear-time.

% \item Conceptual convenience:
% performing a regression involves many experimental choices (e.g. choice of method, kernel, regularization, etc),
% which ideally should be informed by our assumptions and priors
% about the underlying ground-truth $\mu(f)$, such as smoothness, monotonicity, etc.
% It is not always clear how to make these choices, and so the experimenter
% may prefer a tool that does not afford them such choices, and 
% requires minimal assumptions about the data.

% \item Relation to calibration metrics:
% It is easy to read-off a common measure of calibration, the binned ECE,
% from simple visual inspection of the binned reliability diagram.
% \end{enumerate}
% These properties are not always true of more sophisticated methods.


With these desiderata in mind, it is clear that binning leaves room for improvement.
% it is clear that we can likely
% improve upon the method of binning.
As a statistical regression method, binning is rather naive, equivalent to histogram regression.
% and is improved upon in various ways by more sophisticated regressors.
And as a calibration measure, the BinnedECE
% the associated calibration measure of binning, binned-ECE,
has well-known flaws and is sensitive to hyperparameter choices.
We will show how to improve on both aspects:
using a more sophisticated regressor that also corresponds to a consistent calibration measure.
% (Prior work of \citet{UTC1} has formalized what it means for a calibration measure to be ``good'';
% we briefly review it below).
% (We elaborate on what we mean by ``good'' below; we use the notion of a consistent calibration measure from \citet{UTC1}).

% And what is a ``good'' calibration measure?
% Recent theoretical work has identified characteristics
% of good calibration measures
% (including continuity, and tight relations to distance in function space),
% which are captured by the definition of a \emph{consistent calibration measure} \citep{UTC1}.
% Thus, we can hope for regression methods which visually encode
% consistent calibration measures.


\subsection{Our Contributions}
First, we present a construction
of reliability diagrams that (1) implements Nataraya-Watson kernel smoothing as a regression method,
(2) visually encodes a consistent calibration measure (a new measure we call \emph{SmoothECE}),
and (3) is hyperparameter free.

Our theoretical results are more general: we show that kernel-smoothing with essentially any well-behaved
kernel yields a consistent calibration measure. This extends our construction beyond the RBF kernel,
and introduces a new family of consistent calibration measures that are perhaps more intuitive than the ones in \citet{UTC1}.
% This connection even applies if we do the smoothing in ``logit space'', which 
% We prove that 
In fact, this connection extends to general metrics on probabilities in $[0, 1]$:
each metric corresponds to a notion of SmoothECE w.r.t. the metric,
and yields a consistent calibration measure w.r.t. the metric.
For example, we can perform kernel-smoothing in ``logit space,'' which produces
a consistent calibration measure w.r.t. the KL-divergence metric.
% approximates the (lower) distance to calibration 
% Proving this requires 
Technically, proving this requires generalizing the equivalence between \emph{smooth calibration error}
and lower-distance-to-calibration to general metrics \citep{UTC1}.

Finally, we provide a Python package which
computes SmoothECE, and
plots the corresponding kernel-smoothed reliability diagrams.
% It is compatible with scikit-learn, 
It runs in quasilinear-time, and
includes uncertainty quantification via bootstrapping.
We hope this aids adoption of more principled methods in studies of calibration.

\pnote{todo}
{\bf 3. Hyperparameter Free.}
Performing a regression typically involves many experimental choices (e.g. choice of method, kernel, regularization, etc),
which ideally should be informed by our assumptions and priors
about the underlying ground-truth $\mu$, such as smoothness, monotonicity, etc.
However, it is not always clear how to make these choices (such as bin width),
and so we prefer a tool that does not afford us such choices.


% Moreover, methods for uncertainty quantification in regression
% can be directly ported to quantify uncertainty in reliability diagrams
% (e.g. bootstrapping, gaussian process regression, and conformal prediction).

List of contributions (scratch):
\begin{enumerate}
    \item Defining a new consistent calibration measure smECE,
    which has the advantage that it is simple to interpret and visualize. In particular, it closely related to the uncentered-smECE, which is
    simply the ECE of an appropriately smoothed distribution.
    
    Formally: Theorem 1: Let $\smECE^*(f,y)$ be the unique $\sigma^*$ s.t. $\smECE_{\sigma_*}(f,y) = \sigma_*$. Then $\smECE^*$ is a consinstent calibration measure.
    Lemma 4: Let $\smECE^{poor}_{\sigma}$ be non-centered regression stuff. This is equal to $\ECE(f + \sigma \eta, y)$ where $\eta \sim \mathcal{N}(0,1)$. At a scale $\sigma_*$, we have $\smECE^{poor}_{\sigma^*} \approx \smECE_{\sigma_*}$.

    \item This implies a partiularly nice reliability diagram.

    \item smECE is a natural notion of "distance", in the sense that
    small smECE implies a probabilistic post-processing that is near-identity and perfectly calibrated.
    For a given distribution,
    there exists a probabilistic post-processing $\kappa$ such that
    $\E[|f - \kappa(f)|] \leq \smECE$

    \item Explore how far the above results can extend to general metrics.
    First, the definitions extend the defs in UTC1: every metric corresponds to a
    notion of $\smce_d$, and a general notion of lower-calibration distance w.r.t. metric.
    Then, we prove an analgous equivalence as UTC1:
    Theorem 3: (with identical proof as in \cite{UTC1}): $\smce_d \approx \ldce_{d_-}$ where $d_{-}$ is truncation of a metric $d_-(u,v) = \max(d(u,v), 2)$.

    \item Prove analagous result as Theorem 1 in general metrics (with some subtlities).
    Formally, Theorem 4: For an increasing and continuous function $h: [0,1] \to \mathbb{R}\cup \{\pm \infty\}$ (think $h(x) = \log(x/(1-x))$, we define $d_h(u,v) = \max(|h(u) - h(v)|, 2)$, and $\smECE_h$ --- kernel smoothing in the logit space. Then we have $d_h$-consistency of $\smECE_{h}$:  $\ldce_{d_h}(f,y) \leq \smECE_h \leq \sqrt{\ldce_{d_h}}$.
    
    
    \item (Emphasize this part): Moreover, somewhat surprisingly,
    a wide class of general metrics can be related to $\ell_p$ metrics,
    and thus are consistent calibration measures.
    % general metrics can be related to $\ell_p$ metrics under some mild conditions.
    Formally, Theorem 2: if metric $d: [0,1]^2 \to \mathbb{R}$ is well-behaved except the endpoints, then $\smce_d$ is consistent calibration measure.
    This implies that $\smce_d$ w.r.t. the KL metric is a consistent calibratiobn measure.
\end{enumerate}

\subsection{Overview of Techniques}

\pnote{todo: jarek}
The construction is simply: apply Nataraya-Watson kernel smoothing, with a
careful (theoretically-determined) choice of bandwidth.
Notably, the smooth ECE can be read off directly from the reliability diagram,
since it is just the ECE of the kernel-smoothed distribution.
That is, if $\cD$ is the original distribution of prediction-output pairs $(f(x), y)$,
and $\widetilde{\cD}$ is the distribution obtained by 
kernel-smoothing $y$ along $f$, then
\[
\textsf{smECE}(\cD) := \textsf{ECE}(\widetilde{\cD}).
\]
And thus, \textsf{smECE} can be visually computed by looking at deviation from the diagonal
in our smoothed reliability diagram.


{\bf Organization.}
\pnote{todo.}
% We describe the history of reliability diagrams and related works in Section~\ref{sec:related}.
% In Section~\ref{sec:intCE} we present our main method \pnote{which we call...}, a particular type of kernel regression,
% and discuss its theoretical guarantees.
% and include experiments comparing our method to others in Section~\ref{sec:experiments}.



==> intro_code.tex <==
\begin{listing}[t]
\begin{tcolorbox}
\begin{minted}[fontsize=\small]{python}
from relplot import prepare_rel_diagram, plot_rel_diagram, smECE
from sklearn.linear_model import LogisticRegressionCV
from sklearn.datasets import make_classification
from sklearn.model_selection import train_test_split
import relplot.config as rpconfig
rpconfig.use_tex_fonts = True

## generate sample data from logistic regression (via sklearn)
x_train, x_test, y_train, y_test = train_test_split(
                    *make_classification(n_samples = 700, random_state=0),
                    test_size=400, random_state=0)

model = LogisticRegressionCV().fit(x_train, y_train)
f_test = model.predict_proba(x_test)[:, 1]

## plot calibration of model (via our package)
diagram = prepare_rel_diagram(f_test, y_test)
plot_rel_diagram(diagram)
print('calibration error:', smECE(f_test, y_test))
\end{minted}
\end{tcolorbox}
\caption{Example of using our package to generate Figure \ref{fig:hero}.}
\label{listing:1}
\end{listing}


==> math-2.tex <==

For a given kernel $K:[0,1]^2 \to \mathbb{R}$ we define the Kernel smoothing of the residual $r := y-f$ as $y | f$ as
\begin{equation*}
    \hat{r}_K(t) := \frac{\E_{f,y} K(t, f) (y-f)}{\E_{f,y} K(t,f)}.
\end{equation*}

Together with kernel density estimation
\begin{equation*}
    \hat{\delta}(t) := \E_{f} K(t, f).
\end{equation*}
Note that if $K$ is a probability density function of a random variable $\eta$, then $\hat{\delta}$ is a probability density function of a random variable following the law $\eta + f$ (with $\eta, f$ independent).

The $\smECE(f,y)$ is now defined as
\begin{equation*}
    \smECE_K(f,y) := \int |\hat{r}_K(t)| \hat{\delta}_K(t) \dt,
\end{equation*}
which can be simplified to
\begin{equation*}
    \smECE_K(f,y) = \int \left|\E_{f,y} K(t, f) (y-f)\right| \dt.
\end{equation*}

We are focusing on a Gaussian kernel with scale $\sigma$,
\begin{equation*}
    K_{N, \sigma}(x,y) = \frac{1}{\sqrt{2\pi}} \exp(-(x-y)^2/2\sigma^2),
\end{equation*}
and we shall use shorthand $\smECE_\sigma$ to denote $\smECE_{K_{N, \sigma}}$. As it turns out, with this choise of the gaussian kernel we have the monotonicity property: increasing the scale of the smoothing of the residual, decreases the ECE of a smoothed predictions.
\begin{lemma}
    For $\sigma_1 \leq \sigma_2$, we have
    \begin{equation*}
        \smECE_{\sigma_1}(f, y) \leq \smECE_{\sigma_2}(f,y).
    \end{equation*}
\end{lemma}
Note that since $\smECE_{\sigma} \in [0,1]$, and for a given predictor $(f,y)$, the function $\sigma \mapsto \smECE_\sigma(\smECE)$ is a non-increasing function of $\sigma$, there is a unique $\sigma^*$ s.t. $\smECE_{\sigma^*}(f,y) = \sigma^*$.  As we show, this is a convenient scale on which the $\smECE$ of $(f,y)$ should be evaluated. Specifically, we prove the following.
\begin{theorem}
    \label{thm:consistent-intro}
    Let $\smECE^*(f,y)$ be defined as the unique $\sigma^*$ such that $\smECE_{\sigma^*}(f,y) = \sigma^*$. Then $\smECE^*(f,y)$ is a consistent calibration measure.
\end{theorem}

This theorem is a consequence of the following two inequalities. First of all, $\smECE_{\sigma}$ always upper bounds the distance to calibration, if we add the penalty proportional to the scale of the noise $\sigma$.
\begin{lemma}
    For any $\sigma$, we have
    \begin{equation*}
        \ldce(f,y) \lesssim \smECE_\sigma + |\sigma|.
    \end{equation*}
\end{lemma}

On the other hand, as soon as the scale of the noise is sufficiently large compared to the distance to calibration, the $\smECE$ of a predictor is also upper bounded as follows.
\begin{lemma}
Let $(f,y)$ be any predictor Then for any $\sigma$ we have 
\begin{equation*}
    \smECE_{\sigma}(f,y) \leq \left(1 + \frac{1}{\sigma}\right) \ldce(f,y).
\end{equation*}
In particular if $\sigma > 2\sqrt{\ldce}$, then
\begin{equation*}
    \smECE_{\sigma}(f, y) \leq 2 \sqrt{\ldce(f,y)}.
\end{equation*}
\end{lemma}
This lemma, together with the fact that $\sigma \mapsto \smECE_{\sigma}$ is non-increasing implies that the fixpoint satisfies $\sigma^* \leq 2 \sqrt{\ldce(f,y)}$. On the other hand, using the previous inequality, at this fixpoint we have $\ldce(f,y) \leq \sigma^* + \smECE_{\sigma^*}(f, y) = 2 \sigma^*$. That is
\begin{equation*}
    \frac{1}{2} \ldce(f,y) \leq \smECE^*(f,y) \leq 2 \sqrt{\ldce(f,y)},
\end{equation*}
proving the \Cref{thm:consistent-intro}.

\subsubsection{Computation}
For a given $\sigma$, the quantity $\smECE_{\sigma}$ can be efficiently computed, up to a small error $\varepsilon$ in time $\Oh(n + \varepsilon^{-1} \log \varepsilon^{-1})$ in the RAM model.

To this end, we discretize the interval $[0,1]$, splitting it into $M = \lceil \varepsilon^{-1} \rceil$ equal length sub-intervals.
\RestyleAlgo{ruled}
\begin{algorithm}
\KwData{$(f_i, y_i)_{1}^n, M$}
\KwResult{$r$: linear interpolation of $f_i - y_i$ on a grid $[0, 1/M, 2/M, \ldots, 1]$}
%\KwResult{$d$: linear interpolation of density of $f_i$ on a grid $[0, 1/M, 2/M, \ldots, 1]$}
$r \gets \{0\}$\;
\For {$i \in [n]$}{
    $b \gets \lfloor M f_i \rfloor$\;
    $\lambda_{i, b+1} \gets M f_i - b$\;
    $\lambda_{i, b} \gets (1 - \lambda_{i, b})$\;
    $r_b \gets r_b + \lambda_{i,b} (f_i - y_i)$\;
    $r_{b+1} \gets r_{b+1} + \lambda_{i, b+1} (f_i - y_i)$\;
%    $d[b] \gets d[b] + \frac{1 - \lambda}{n}$\;
%    $d[b+1] \gets d[b] + \frac{\lambda}{n}$\;
%    \return{$r, d$}
}
\caption{Discretization} \label{alg:disc}
\end{algorithm}

\begin{algorithm}
\KwData{$(f_i, y_i)_{1}^n, \sigma, \varepsilon$}
\KwResult{$\smECE_\sigma(\{(f_i, y_i)\})$}
$r, d \gets \text{Discretization}(\{f_i, y_i]\}, \lceil \varepsilon^{-1} \rceil$\;
$K \gets \mathrm{DiscreteGaussianKernel}(\sigma, \lceil \varepsilon^{-1}\rceil)$\;
$\tilde{r} \gets r \ast K$\;
$S \gets \sum_i |\tilde{r}[i]|$\;
$\textbf{return}\ S$\;
\caption{Efficient estimation of $\smECE$} \label{alg:convolution}
\end{algorithm}

The discretization method (\Cref{alg:disc}) runs in time $\Oh(n)$ (assuming random access to the memory of size $\Oh(\varepsilon^{-1})$), and produces a linear interpolation for the residuals $r_i - f_i$. Specifically, it outputs an array $r$, s.t.
\begin{equation*}
    r_t := \sum_{i \in [n]} \lambda_{i, t} (y_i - f_i),
\end{equation*}
where $\lambda_{i,t} := \max( 1 - M |f_i - t/M|, 0)$.

The method $\smECE$ then proceeds to compute convolution $r \ast K$ with the discretization of the Gaussian kernel probability density function, i.e. $\tilde{K}_t := \exp(-t^2/2\sigma^2)$, and $K_t := \tilde{K}_t \left / \sum_i \tilde{K}_t \right.$

This convolution $\tilde{r} := f \ast K$ can be computed in time $\Oh(M \log M)$ using a fast fourier transform, and is implemented in a majority of mathematical libraries. Finally, we report the sum of absolute values of the residuals $\sum |\tilde{r}_i|$.

==> overview.tex <==
\subsection{Overview of Tecniques}
\pnote{todo -- jarek}

==> prelim.tex <==
\section{Notation and Preliminaries}

\jnote{I'm not sure where this should go...}
For a metric space $(\cX, d)$, let us consider $\Delta(\cX)$ to be the space of all probability distributions over $\cX$. We define the \emph{Wasserstein} metric on the space $\Delta(X)$ (sometimes called Earth-movers metric). \jnote{Add citation}

\begin{definition}[Wasserstein distance]
For two distributions $\mu, \nu \in \Delta(\cX)$ we define the Wasserstein distance
\begin{equation*}
    W_1(\mu, \nu) := \inf_{\gamma \in \Gamma(\mu,\nu)} \E_{(x,y) \sim \gamma} d(x,y),
\end{equation*}
where $\Gamma(\mu, \nu)$ is a family of all couplings of distributions $\mu$ and $\nu$.
\end{definition}

\iffalse
\begin{definition}
    A distribution $\cD$ over $[0,1] \times \{0, 1\}$ of a prediction $f$ and outcome $y$ is \emph{perfectly calibrated} if 
    \begin{equation*}
        \E[y|f] = f.
    \end{equation*}
\end{definition}

\begin{definition}[Perfect calibration]
For a distribution $\cD$ over $[0,1] \times \{0,1\}$ of pairs prediction and outcome, 
the $\ldce(\cD)$ is defined as a Wasserstein distance to the nearest perfectly calibrated distribution.

We say that a map $\mu : \Delta([0,1] \times \{0, 1\} \to \mathbb{R}_+$ is a \emph{consistent calibration measure} if it is polynomially upper and lower bounded by $\ldce$. That is, if there exists $c_1, c_2, \alpha_1, \alpha_2$ such that for any $\cD$
\begin{equation*}
    c_1 \ldce(\cD)^{\alpha_1} \leq \mu(\cD) \leq c_2 \ldce(\cD)^{\alpha_2}.
\end{equation*}
\end{definition} 
\fi

% At this point,
% it is helpful to introduce some notation.
% We have a binary classifier $f$ producing probabilities $f(x) \in [0, 1]$.
% We are given iid samples of prediction and observation pairs:
% $\{(f(x_i), y_i)\}_{(x_i, y_i) \sim \cD}$ where $y_i \in \{0, 1\}$.
% For example, the rain forecast $f(x_i)$ and
% the corresponding actual observation of rain $y_i \in \{0, 1\}$.
% The true conditional density function (the regression function) is
% $\mu(\ell) := \E_{(x, y) \sim \cD}[ y \mid f(x)=\ell]$.
% The plot of our estimate of $\mu: [0, 1] \to [0, 1]$ is
% sometimes called an ``ideal reliability diagram'' --- though it will not be ideal for us.
% A perfectly calibrated classifier will have $ \mu(\ell) = \ell$,
% and thus a diagonal regression function.

% With the above setup, it is clear that 
% constructing a reliability diagram is simply a 1-dimensional regression problem.
% After all, our goal is to estimate the conditional $\mu(f) = \E[y \mid f]$
% given iid samples $(f_i, y_i) \in \R \x \R$, where we let $f_i := f(x_i)$.
% This is exactly the objective of regressing $y \in \R$ on $f \in \R$.
% Thus, all regression methods yield a corresponding method of constructing reliability diagrams:
% the popular practice of ``binning'' reliability diagrams, for example,
% exactly corresponds to the histogram-estimator in statistics,
% which fits a family of piecewise-constant functions to $\mu(f)$.

==> recalibration.tex <==
\section{Reliability Diagrams and Recalibration}
\pnote{Actually, just say a few sents about this in a discussion.}
TODO.

There is close connection between reliability diagrams and recalibration.
Any method that produces a function $T(f)$ estimating $\E[ y \mid f]$
can be used as a ``recalibration'' method: post-processing as $(T \circ f)$
re-calibrates the classifier $f$, hopefully to something with smaller calibration error\footnote{Whether it is actually closer to calibrated depends on the details of the method.}.
We thus expect that methods commonly used for post-processing-based
recalibration (e.g. logistic regression)
will also work well as reliability diagrams.
\jnote{Wait, what?!}

Note that a perfect reliability diagram (perfect estimate of $\E[ f | y]$) 
yields a perfect re-calibrator, but not vice versa (e.g. consider the constant function as a recalibrator).

==> regression.tex <==
\section{Reliability Diagrams from Regression Methods}
\label{sec:generic}
\pnote{todo, remove most/all this}
We briefly review how to use a generic regression method to produce a reliability diagram.
% There is nothing new here besides simply doing the regression --- we are just being explicit
% about certain regression best-practices (such as using a validation set to find hyperparameters).
% There is nothing new about this method; it simple apples best-practices from regression
% (such using a validation to find optimal hyperparameters).
% We present the specific case of using Nataraya-Watson kernel smoothing, but any regression method would suffice.
For concreteness, we present this using Natarya-Watson kernel regression,
but any regression method can be substituted.
% because it has favorable theoretical properties (see Section~\ref{?}),

% the user is free to choose their favorite regression method.

\begin{enumerate}
    \item Split samples $\{(f(x_i), y_i)\} \equiv \{(f_i, y_i)\}$ into a train set $S$ and holdout set $H$.
    \item Let $\hat{\mu}_\lambda$ be the Nataraya-Watson kernel regression estimate of $y$ given $f$ 
    on the train set $S$, using a triangular kernel with bandwidth $\lambda$. That is,
    \[
        \hat{\mu}_\lambda(f) :=
        \frac{\sum_{(f_i, y_i) \in S} y_i K_\lambda(f-f_i)}{\sum_{(f_i, y_i) \in S} K_\lambda(f-f_i)}
    \]
    where $K_\lambda(x) := \lambda^{-1}\textrm{ReLU}(1-\lambda^{-1}x)$ is the triangular kernel.
    \item Chose optimal hyperparameters $\lambda^*$ by minimizing the $\mathcal{L}_2$ loss (or any other proper loss) on the holdout set:
    \[
    \lambda^*
    = \argmin_\lambda \mathcal{L}(\hat{\mu}_\lambda)
    = \argmin_\lambda \sum_{(f_i, y_i) \in H} ||\hat{\mu}_\lambda(f_i) - y_i||^2
    \]
    \item Output $\hat{\mu}_{\lambda^*} : [0, 1] \to [0, 1]$ as the reliability diagram.
\end{enumerate}

There is nothing new here besides simply doing the regression --- we are just being explicit
about certain regression best-practices (such as using a validation set to find hyperparameters).
\pnote{add footnote on logloss being MLE}

\paragraph{Implementation Notes.}
We suggest several practical improvements:
Perform the regression on centered targets $(y_i - f_i)$ instead of the original targets $y_i$,
since many regression methods assume centered priors.
Also, use cross-validation to find optimal hyperparameters
(instead of a single train/holdout split), 
and report confidence bands on the regression via bootstrapping.
Finally, we specifically suggest using Natarya-Watson kernel regression with the triangular kernel,
due to its favorable theoretical properties (see Section~\ref{?}). In this case,
there is a better way to choose the kernel bandwidth than cross-validation,
as we describe in Section \ref{?}.
We implement these suggestions in the provided code \ref{?}, which produces diagrams such as Figure~\ref{fig:hero}

\paragraph{Importance of Cross-Validation}
For most regression methods, it is important to pick regression hyperparameters
by optimizing for the \emph{test loss},
as estimated e.g. by cross-validation, to avoid overfitting.
In particular, if binning must be used, one should at least choose the width of bins
to minimize the regression test loss.
This strategy for picking bin-widths implicitly addresses the common concerns with binning:
it balances the approximation-error from picking too large bins
with the generalization-error from picking too small bins.
After all, these are the same concerns we have in regression.
This strategy has been suggested before \citep{brocker2008some},
though it does not appear to be well known in the calibration literature.



